FEAST Eigenvalue Solver v3.0 User Guide

The FEAST eigensolver package is a free high-performance numerical library for solving the Hermitian and non-Hermitian eigenvalue problems, and obtaining all the eigenvalues and (right/left) eigenvectors within a given search interval or arbitrary contour in the complex plane. Its originality lies with a new transformative numerical approach to the traditional eigenvalue algorithm design - the FEAST algorithm. The FEAST eigensolver combines simplicity and efficiency and it offers many important capabilities for achieving high performance, robustness, accuracy, and scalability on parallel architectures. FEAST is both a comprehensive library package, and an easy to use software. It includes flexible reverse communication interfaces and ready to use predefined interfaces for dense, banded and sparse systems. The current version v3.0 of the FEAST package can address both Hermitian and non-Hermitian eigenvalue problems (real symmetric, real non-symmetric, complex Hermitian, complex symmetric, or complex general systems) on both shared-memory and distributed memory architectures (i.e contains both FEAST-SMP and FEAST-MPI packages). This User's guide provides instructions for installation setup, a detailed description of the FEAST interfaces and a large number of examples.

==> feast_customcontour.tex <==
\section{Custom Contours with FEAST}

Only eigenvalues inside of the user defined interval are calculated with FEAST.  Since eigenvalues of Hermitian (and real-symmetric) matrices are real this interval can be defined by [$\lambda _{min}$, $\lambda _{max}$]. Non-Hermitian matrices possess a complex eigenspectrum and require a 2-dimensional interval. The Custom Contour feature grants the flexability to target specific eigenvalues. This feature is available for both Hermitian and non-Hermitian codes and must be used with "Expert" routines that take two additional arguments containing the complex integration nodes and weights. Custom contours can be employed by following three simple steps: (1) Define contour, (2) Calculate corresponding integration nodes and weights, and (3) Call "Expert" FEAST routine (either driver or RCI).

%\vspace{2mm}
%\begin{small}
%\begin{tabular}{r l}
%1. & Define contour \\
%2. & Calculate corresponding integration nodes and weights \\
%3. & Call "Expert" FEAST routine (either driver or RCI) \\
%\end{tabular}
%\end{small}

\subsection{Defining a Custom Contour}

Users can must only define the geometry of their contour. The contour can be comprised of line segments and half ellipses. Two important points to note: {\bf the actual contour is a polygon} defined by the integration points along the path - and - {\bf only convex contours may be used}. A contour is defined using the following three arrays.

\vspace*{2mm}
\hrule
\begin{small}
\begin{itemize}
\vspace*{-1mm}
\itemsep0pt
	 \item[1.] {\bf Zedge}(1:ccN) - Complex endpoints of each contour piece
	 \vspace{-2mm}
	 \begin{itemize}
	 \itemsep0pt
	 	\item [$\bullet$] Pieces must be specified in order and in the clockwise direction.
		 \item [$\bullet$] The $k^{th}$ piece is be specified by its 2 endpoints contained in Zedge($k$) and Zedge($k+1$). It is assumed that the last piece is connected to the first.
 	 \end{itemize}
	 \vspace{-2mm}
	 \item[2.] {\bf Tedge}(1:ccN) - The type of each contour piece \\
	  \textit{Line:} \hspace{5.2mm} Tedge($k$) $=$ 0 \\
	  \textit{Ellipse:} \hspace{2mm}  Tedge($k$) $\neq$ 0 (specifies the 2nd radius)\\
	  \hspace*{15mm} If (Tedge($k$) $>$ 0) $r_s = r_p*Type$ \hspace*{10.7mm} - $r_p$ is calculated from the endpoints \\
	  \hspace*{15mm} If (Tedge($k$) $<$ 0) $r_s = r_p / abs(Type) $ \hspace{5mm} - $r_s$ is secondary radius  \\
	  %\hspace*{15mm} - $r_p$ is calculated from the endpoints \\
	  %\hspace*{15mm} - $r_s$ is secondary radius \\
	  \hspace*{15mm} Note: $Type= \pm 1$ creates a half circle \\
          \vspace{-5mm}
	  \item[3.] {\bf Nedge}(1:ccN)	- Then integration accuracy for each piece
	  \vspace{-2mm}
	  \begin{itemize}
	  \itemsep0pt
	 \item [$\bullet$] The number of intervals for the trapezoidal integration along each contour piece. 
	  \end{itemize}	 	
	 \vspace{-2mm}
	  \item[4.] {\bf ppN} = SUM({\bf Nedge}(1:ccN)) -  The total number of integration nodes.
\end{itemize}
\hrule
\end{small}

\subsection{Calculating Integration Nodes and Weights}
We have provided a companion routine \texttt{[cz]feast$\_$customcontour} that will automatically populate the two additional arrays, $Zne$ and $Wne$, needed as inputs to FEAST. A F90 code snippet to generate a contour (seen in \ref{fig_customcontour} ) is given below. See {\bf Chapter 6} for more details on the argument list of this function. 
\noindent
%\begin{minipage}{0.6\textwidth}
\begin{small}
\begin{lstlisting} [frame=trBL]
!!! Example contour - Figure 5.1 (rs = 0.5*r)
call feast_init(fpm)
ccN = 3 ! number of pieces that make up contour 
allocate( Zedge(1:ccN),Nedge(1:ccN),Tedge(1:ccN) )
Zedge = (/(0.0d0,0.0d0),(0.0d0,1.0d0),(6.0d0,1.0d0)/)
Tedge(:) = (/0,0,-2/)
Nedge(:) = (/8,8,8/)
fpm(2) = sum(Nedge(1:ccN)) !!User enter # of contour points
allocate( Zne(1:fpm(2)), Wne(1:fpm(2)) ) 
call zfeast_customcontour(fpm,ccN,Nedge,Tedge,Zedge,Zne,Wne)
\end{lstlisting}	
\end{small}  
%\end{minipage}\hfill
%\begin{minipage}{0.3\textwidth}
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth,angle=0]{CustomContour2.pdf}
\caption{Example contour containing two line segments (pieces 1 and 2) and a half ellipse (piece 3). The secondary radius is half of the primary radius defined by nodes a and b. }
\label{fig_customcontour}
\end{figure}
%\end{minipage}


\subsection{Calling the Expert Routine}

There exists an expert version of each FEAST driver and RCI routine. They are signified by an appending ``x" and accept the two additional arguments $Zne$ and $Wne$ containing the integration nodes and weights. Below is an example F90 code calling the dense general complex FEAST driver with a custom contour.

\begin{small}
\begin{lstlisting} [frame=trBL]
program feast_cc
  complex(kind=kind(1.0d0)),dimension(:,:),allocatable :: A, B, X
  complex(kind=kind(1.0d0)),dimension(:),allocatable :: E, Zne, Wne, Zedge
  complex(kind=kind(1.0d0)) :: Emid 
  double precision :: r, epsout
  integer :: M0, ccN, info, M, N, LDA, LDB
  integer,dimension(64) :: fpm
  double precision,dimension(:),allocatable :: res
  integer,dimension(:),allocatable :: Nedge, Tedge

   allocate(A(1:N,1:N), B(1:N,1:N), E(1:M0), X(1:N,1:2*M0), res(1:2*M0))
   ... Load A,B
   call feastinit(fpm)
   ... Define Custom Contour - Fill Zedge,Tegde,Nedge
   fpm(2) = sum(Nedge(1:ccN))
   allocate( Zne(1:fpm(2)), Wne(1:fpm(2)) ) 
   call zfeast_customcontour(fpm(2),ccN,Nedge,Tedge,Zedge,Zne,Wne)
   call zfeast_gegvx(N,A,LDA,B,LDA,fpm,epsout,loop,
                         Emid,r,M0,E,X,M,res,info,Zne,Wne)
end program feast_cc
\end{lstlisting}	
\end{small}   
	 


